Class-relation Knowledge Distillation for Novel Class Discovery

We tackle the problem of novel class discovery, which aims to learn novel classes without supervision based on labeled data from known classes. A key challenge lies in transferring the knowledge in the known-class data to the learning of novel classes. Previous methods mainly focus on building a shared representation space for knowledge transfer and often ignore modeling class relations. To address this, we introduce a class relation representation for the novel classes based on the predicted class distribution of a model trained on known classes. Empirically, we find that such class relation becomes less informative during typical discovery training. To prevent such information loss, we propose a novel knowledge distillation framework, which utilizes our class-relation representation to regularize the learning of novel classes. In addition, to enable a flexible knowledge distillation scheme for each data point in novel classes, we develop a learnable weighting function for the regularization, which adaptively promotes knowledge transfer based on the semantic similarity between the novel and known classes. To validate the effectiveness and generalization of our method, we conduct extensive experiments on multiple benchmarks, including CIFAR100, Stanford Cars, CUB, and FGVC-Aircraft datasets. Our results demonstrate that the proposed method outperforms the previous state-of-the-art methods by a significant margin on almost all benchmarks. Code is available at \href{https://github.com/kleinzcy/Cr-KD-NCD}{here}.

==> conclusion.tex <==
\section{Conclusion}
% 本文中，我们提出了一个novel class-relation knowledge distillation learning framework, which provides a new perspective to transfer knowledge from known to novel clases for the NCD community. Instead of transferring knowledge only by sharing representation space, we utilize class relations to transfer knowledge. In particular, 我们观察到novel classes在known classes训练地模型上响应，能够很好的表示novel classes与known classes之间的关系，但是，这种关系在discovery traing phase被破坏了。因此，为了保持这种meaningful的类间关系，我们提出了一个简单有效的regularization term，它约束discovery training phase的模型，保持原来的关系。并且，我们提出一个可学习的权重函数，它动态地分配更多的权重给语义相近的样本，使模型学习共享的语义信息。我们在几个通用数据集，和几个fine-grained dataset上都取得了明显的提升，验证了我们方法的有效性。此外，我们希望我们的发现，能够shed more light on futre work to explore the relation between known and novel classes, and enhance the models transferbility.

In this paper, we propose a novel class-relation knowledge distillation learning framework, which provides a new perspective to transferring knowledge from known to novel classes in the NCD problem. Instead of transferring knowledge only by sharing representation space, we utilize class relations to transfer knowledge. Specifically, we observe that the prediction distribution of novel classes on a model trained on known classes effectively captures the relationship between the novel and known classes. However, this relationship is disrupted during the discovery training stage. Therefore, to maintain this meaningful inter-class relationship, we propose a simple and effective regularization term that constrains the model in the discovery training stage. Additionally, we propose a learnable weight function that dynamically assigns more weight to semantically similar samples, enabling the model to learn the shared semantic information. Our method achieves significant improvements on several general datasets and fine-grained datasets, validating the effectiveness of our approach. Furthermore, we hope our findings will shed more light on future work to explore the relationship between known and novel classes and enhance the model's transferbility for knowledge transfer.

\section*{Acknowledgement}
This work was supported by Shanghai Science and Technology Program 21010502700, Shanghai Frontiers Science Center of Human-centered Artificial Intelligence and MoE Key Lab of Intelligent Perception and Human-Machine Collaboration (ShanghaiTech University).
